Topology of Bands in Solids : From Insulators to Dirac Matter

Bloch theory describes the electronic states in crystals whose energies are distributed as bands over the Brillouin zone. The electronic states corresponding to a (few) isolated energy band(s) thus constitute a vector bundle. The topological properties of these vector bundles provide new characteristics of the corresponding electronic phases. We review some of these properties in the case of (topological) insulators and semi-metals.

==> bourbaphydefs.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Begin of definition file AHPEFS.TEX                      %
% (c) Stephan Ammann, for Birkhaeuser, Dec 1999            %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% AHPDEFS.tex -- is red in by each header file             %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\font\fxtit=cmssbx10 % For the new logo

\newcount\fpage\newcount\npage\newcount\lpage
\fpage=\fipage\npage=\nrpage
\lpage=\fpage\advance\lpage by\npage\advance\lpage by-1

\def\xrule{\vrule width2.25pt}
\def\yrule{\hrule height.5pt}
\def\yrulefill{\leaders\yrule\hfill}
\def\strutx{\vrule height8.5pt width0pt depth0pt}
\def\struty{\vrule depth3.5pt width0pt}
\def\strutz{\vrule height10.2pt width0pt}

\def\boxl{\vbox{\halign{##\hfil\cr
S{\'e}minaire Poincar{\'e} \volnr\ (\centnr\yearnr)  
\the\fpage\ -- \the\lpage\cr
%\struty \copyright\ Birkh{\"a}user Verlag, Basel,
%\centnr\yearnr\cr
%1424-0637/\yearnr/\issuenr0\fipage-\the\npage\ \ %
%\$\,1.50$+$0.20/0\cr
}}}


\def\boxr{\vbox{\offinterlineskip
\halign{##\hfil\hskip1mm&##\hfil\cr
\noalign{\vskip.8mm}
\multispan2{\yrulefill}\cr
\xrule\strutz\struty
&\fxtit S{\'e}minaire Poincar{\'e}\cr
%\xrule\strutx&%
%\vbox to0pt{%
%\vbox to0pt{\vss\hbox{\fxtit and Applications NoDEA}}\vss}\cr
}}}

\def\titlebox{\vbox to0pt{\hsize=150mm\footnotesize\vss
\hbox to\hsize{\boxl\hfil\boxr}}}


\def\ps@myheadings{
\let\@mkboth\markboth
\def\@oddhead{\footnotesize \rm Vol. \volnr, \centnr\yearnr
\hspace{6mm}\titletxt\hfil\thepage}%
\def\@oddfoot{} % % centered page number
\def\@evenhead{\footnotesize \thepage \hfil
\authortxt\hspace{6mm}S{\'e}minaire Poincar{\'e}}%
\def\@evenfoot{}%       % centered page number
}

\def\ps@plain{
\let\@mkboth\markboth
\def\@oddhead{%
\titlebox}%
\def\@oddfoot{}%      % centered page number
\def\@evenhead{}%
\def\@evenfoot{}%     % centered page number
}

\ps@myheadings              % 'myheading' page style
\pagenumbering{arabic}      % Arabic page numbers
\onecolumn                  % Single-column.

\setcounter{page}{\fpage}

\textwidth=150mm
\textheight=230mm
\parindent=8mm
\evensidemargin=0pt
\oddsidemargin=0pt
\topmargin=0pt
\frenchspacing

\newcommand{\pdpg}{\postdisplaypenalty=-2000}
%% Used to force a page-break after a displayed equation

\let\dst=\displaystyle
\let\scr=\scriptstyle

\def\bfdefault{b}

\def\Rec{Received\ }
\def\Rev{Revised\ }

\endinput

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% End of AHPDEFS.TEX                                       %
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
% End of definition file

%%% Local Variables: 
%%% mode: plain-tex
%%% TeX-master: t
%%% TeX-master: t
%%% TeX-master: t
%%% End: 


==> carpentier_h.tex <==
\def\BZ{\ensuremath{\text{BZ}}}
\def\dd{\ensuremath{\mathrm{d}}}
\def\ee{\ensuremath{\mathrm{e}}}
\def\ii{\ensuremath{\mathrm{i}}}

\def\can{\ensuremath{\text{can}}}
\def\std{\ensuremath{\text{std}}}

\def\un{\ensuremath{\text{I}}}
\def\deux{\ensuremath{\text{II}}}
\def\unA{\ensuremath{\text{IA}}}
\def\unB{\ensuremath{\text{IB}}}

